COME: Test-time adaption by Conservatively Minimizing Entropy

Machine learning models must continuously self-adjust themselves for novel data distribution in the open world. As the predominant principle, entropy minimization (EM) has been proven to be a simple yet effective cornerstone in existing test-time adaption (TTA) methods. While unfortunately its fatal limitation (i.e., overconfidence) tends to result in model collapse. For this issue, we propose to Conservatively Minimize the Entropy (COME), which is a simple drop-in replacement of traditional EM to elegantly address the limitation. In essence, COME explicitly models the uncertainty by characterizing a Dirichlet prior distribution over model predictions during TTA. By doing so, COME naturally regularizes the model to favor conservative confidence on unreliable samples. Theoretically, we provide a preliminary analysis to reveal the ability of COME in enhancing the optimization stability by introducing a data-adaptive lower bound on the entropy. Empirically, our method achieves state-of-the-art performance on commonly used benchmarks, showing significant improvements in terms of classification accuracy and uncertainty estimation under various settings including standard, life-long and open-world TTA, i.e., up to $34.5\%$ improvement on accuracy and $15.1\%$ on false positive rate.

==> sections/EM.tex <==
\section{The Greedy nature of Entropy minimization}
In this section, we hypothesis that continuously pursuing low uncertainty which is the instinct nature of EM, can be harmful to the model representation ability and trustworthiness, as we demonstrate both empirically and theoretically. Along the same testing trajectory, the predictive confidence increases quickly from the initial model (as measured by the maximum of softmax probability), after which the model start to be overconfident on even wrong predictions. At the same time, the model classification performance improves temporarily for very short time horizon before quickly dropping.

We attribute the catastrophic collapse in term of classification performance and trustworthiness to the greedy nature of the EM algorithm due to the fact that it minimizes the predictive entropy. 



==> sections/method.tex <==
\section{Uncertainty-aware Entropy Minimization}
We introduce uncertainty-aware entropy minimization (UEM), a simple alternative beyond EM algorithm. The key idea of UEM is to accurately quantify and regularize the model uncertainty during TTA progress, and thus avoid the greedy nature of EM and further improve the TTA performance. We first introduce uncertainty quantification by the theory of evidence which is the the fundamental block of UEM and then present how to regularize the uncertainty during TTA.

\subsection{Modeling uncertainty by the Theory of Evidence}
Subjective logic (SL)~\cite{jsang2018subjective} is a Bayesian framework for uncertainty quantification. Non-Bayesian classifiers consider the model's output $f(x)$ as logits, which is then normalized with softmax to directly model predictive categoricals $p(\hat{y}|x)$. While in Bayesian framework~\cite{malinin2018predictive}, $f(x)$ is used for parameterize a Dirichlet distribution $p(\mu|x)$ firstly, which models the prior of all possible categoricals $\mu$ by
\begin{equation}
\label{dirichlet}
    p(\mu|x)={\rm Dir}(\mu|\boldsymbol{\alpha})=\frac{\Gamma(\alpha_0)}{\prod_{k=1}^K\Gamma(\alpha_k)}\prod_{k=1}^K \mu^{\alpha_k-1}_k, \ \boldsymbol{\alpha}= \exp {\rm ReLU}(f(x)),
\end{equation}
where ${\rm Dir}(\mu|\boldsymbol{\alpha})$ is Dirichlet distribution and $\boldsymbol{\alpha}$ is the concentration parameters of Dirichlet. The sum of all $\alpha_k\in\boldsymbol{\alpha}$ is so called the strength $S$ of the Dirichlet distribution, i.e., $S=\sum_{k}\alpha_k$. In Eq.~\ref{dirichlet}, the ReLU and Exp function is employed to ensure $\forall \alpha_k\in \boldsymbol{\alpha},\alpha_k\geq1$, which is an requirement for valid parameters of a Dirichlet distribution. SL allows one to use the principles of evidential theory to quantify belief masses and \textit{uncertainty}. First, SL connects the parameters of the Dirichlet $\boldsymbol{\alpha}$ to \textit{evidence} $e$ by $\boldsymbol{\alpha}=\boldsymbol{e}+1$. Noted that the \textit{evidence} in Bayesian context refers to the metrics collected from the input to support the classification. Once collected evidence, SL assigns the brief masses $b$ of each class label and uncertainty mass $u$ to the whole frame based on evidence as follow
\begin{equation}
\label{SL}
    b_k=\frac{e_k}{S}=\frac{\alpha_k-1}{S}\ {\rm and} \ u=\frac{K}{S}, \ {\rm subject\ to} \ u+\sum_{k=1}^K b_k =1 
\end{equation}
where $S$ is the Dirichlet strength which denotes the total evidence we collected and $K$ is the classes number. Eq.~\ref{SL} actually describes the phenomenon where the more evidence observed for the $k$-th category, the greater the brief mass assigned to the $k$-th class. Correspondingly, the less total evidence $S$ observed, the greater the total uncertainty $u$. Once given such brief assignment (i.e., opinion), the final prediction is the mean of the corresponding Dirichlet distribution which can be computed as
\begin{equation}
    \hat{\mu} =\mathbb{E}_{\mu}{\rm Dir}(\mu|\alpha)=\frac{\boldsymbol{\alpha}}{S}.
\end{equation}

\subsection{Uncertainty-aware model adaption}
UEM explicitly exploits the uncertainty information to mitigate the greedy nature of EM. Specifically, vanilla EM minimize the softmax entropy of the predicted class distribution, which inevitably results in assigning rather high probability to one certain class. In contrast, our UEM first constructs the opinion $\mathcal{M}$ based on SL as follow
\begin{equation}
    \mathcal{M}(x)=[b_1,b_2,\cdots,b_k,u],
\end{equation}
where $\mathcal{M}(x)$ explicitly models the uncertainty due to lack-of-evidence. Then instead of enforcing the model classify $x$ into one certain class belongs to $\{1,\cdots,K\}$, we offer the model with an additional option, i.e., present high overall uncertainty and reject to classify when the observed total evidence is insufficient. Specifically, we conduct entropy minimization on the opinion $\mathcal{M}(x)$ by
\begin{equation}
    \underset{\theta}{\rm minimize}\  H(\mathcal{M}(x))=-\sum_{k=1}^K b_k\log b_k-u\log u
\end{equation}
\textbf{Advantages of considering model output as subjective opinions.} Compared to EM with softmax entropy, using subjective uncertainty is more suitable for model adaption in the wild environment, where there always exists irreducible uncertainty raised from abnormal outliers or class overlap which cannot diminish in unsupervised model adaption process. Subjective logic provides an additional uncertainty mass function $u(x)$ that allows the model distinguish between a lack of evidence. Instead of enforcing low uncertainty on all test samples, our UEM only encourage the model to make a sharp prediction, whether classify $x$ to certain class belong to $\{1,\cdots,K\}$ or reject it with high uncertainty. Besides, compared to existing works which need to modify the original model architecture to identify outliers, our UEM is model-agnostic can be applied to any pretrain model (e.g., huggingface, torchvision), which is more suitable for the TTA setting.

\subsection{Enhancing uncertainty by additional regularization}
Still subjective entropy minimization offers an opportunity to modeling uncertainty and reject to classify unreliable samples, it has been shown experimentally that the uncertainty estimated in this way may not be ideal enough without additional regularization. To address this, we propose to employ the uncertainty information provided the pretrain model to enhance the uncertainty estimation. More specifically, we constrain the uncertainty mass predicted by the adapted model to not diverge far from the pretrain model. This results in the following constrained optimization objective
\begin{equation}
\label{constrained-op}
    \underset{\theta}{\rm minimize}\  H(\mathcal{M}(x))\ \ {\rm subject\ to}\ |u_{\theta}(x)-u_{\theta_0}(x)|\leq \delta
\end{equation}
where $\theta$, $\theta_0$ denote the adapted and pretrain model respectively, $u$ is the uncertainty estimated by Eq.~\ref{SL} and $\delta$ is a threshold.

Considering the difficulty of constrained optimization in modern neural networks, our next target is to find a way to convert Eq.~\ref{constrained-op} into an unconstrained form. To this end, we introduce the following Lemma
\begin{theorem} For any $x\in\mathcal{X}$, we have
    \begin{equation}
      -||x||_{p}\leq \log  u(x)\leq  \log K-K^{-1/p}||x||_p
    \end{equation}
\end{theorem}



Noted that the uncertainty mass function is in essence depended on the strength of Dirichlet $S$
\begin{equation}
   u(x)\propto K/S, \ {\rm where}\ S=\sum_{k=1}^K \alpha_k=\exp^{{\rm LSE}({\rm ReLU}(f))}
\end{equation}
where ${\rm LSE}(\cdot)$ denotes the logsumexp function. Thus we can explicitly constrain on $u_{\theta}(x)$ by removing the gradient on ${\rm LSE}({\rm ReLU}(f))$ during optimization with gradient descent algorithm. The final minimizing objective is
\begin{equation}
   \underset{\theta}{\rm minimize}\  H(\mathcal{M}(x))\ \ {\rm where}\ f_k = \frac{{\rm ReLU}(f_k)}{{\rm LSE}({\rm ReLU}(f))}\cdot{\rm LSE}({\rm ReLU}(f)).detach()
\end{equation}
where $detach()$ means removing gradient which is a common used function in modern deep learning toolbox like PyTorch and TensorFlow. Our UEM can be implemented by modifying only a few lines of code in the original EM algorithm.


\begin{algorithm}[H]
\caption{Pseudo code of UEM in a PyTorch-like style.}
\begin{minted}{python}
# x: the output logits
# model: the test model

def subjective_logic_entropy(x):
    x = torch.ReLU(x) # ensure x greater than zero
    x = x/logsumexp(x)*logsumexp(x).detach() # uncertainty constrain
    brief = exp(x)/(sum(exp(x))+K) # brief mass
    uncertainty = K/(sum(exp(x))+K) # uncertainty mass
    opinion = cat([brief,uncertainty]) # subjective opinion
    return -sum(opinion*log(opinion)) # entropy of opinion

for data in test_loader: # load a minibatch data
    x = model(data) # forward
    loss = subjective_logic_entropy(x) # calculate loss
    loss.backward() # take gradients
    
\end{minted}
\end{algorithm}


==> sections/preliminaries_v2.tex <==
\section{Preliminaries}
\textcolor{blue}{We consider the fully test-time adaption setting in $K$-classification task where $\mathcal{X}$ is the input space and $\mathcal{Y}=\{1,2,...,K\}$ denotes the target space. Given a classifier $f:\mathcal{X}\rightarrow \mathbb{R}^K_{+}$ parameterized by $\theta$ which has been pretrained on training distribution $P^{\rm train}$, our goal is to boost $f$ by updating its parameters $\theta$ online on each batch of test data drawn from test distribution $P^{\rm test}$. Note that in fully TTA setting, the training data $P^{\rm train}$ is inaccessible and one can only tune $\theta$ on unlabeled test data. This is derived from realistic concerns of privacy, bandwidth or profit.
\textbf{Entropy minimization (EM)} algorithm iteratively optimizes the model to minimize the predictive entropy on test sample $x$
\begin{equation}
    H(p(y|x))=-\sum_{k=1}^K p(y=k|x)\log p(y=k|x),
\end{equation}  
where $p(y|x)$ is the class distribution calculated by normalizing the output logits $f(x)$ with softmax function, i.e.,  $p(y=k|x)=\frac{\exp f_k(x)}{\sum \exp f(x)}$. $H$ is the Shannon's entropy.}


\textcolor{blue}{\textbf{Other learning objectives.} Besides EM, there also exists several TTA methods which explore other unsupervised learning objectives. Notable examples include 1) Pseudo label (PL): $\mathcal{L}_{\rm PL}=-\mathbb{E} \log p(y=\hat{y}|x)$ which encourages the adapted model to fit the pseudo label $\hat{y}$ predicted by the pretrained model, 2) Module adjustment (T3A) which adjusts the parameters in the last fully connected layer, and can be viewed as an implicit way to minimize entropy~\citep{iwasawa2021test}, 3) Energy minimization: 
$\mathcal{L}_{\rm TEA}=-\mathbb{E} \log\sum_{k=1}^K \exp f(x)$ which aims to minimize the free energy during adaption, and takes inspiration from energy model~\citep{yuan2023energy}, 4) Contrastive learning objective: $\mathcal{L}_{\rm infoNCE}=-\log \frac{\exp {\rm query}\cdot {\rm key^{+}}}{\sum \exp {\rm query}\cdot {\rm key}}$ which strives to minimize the cosine distance between the query and positive samples ($\rm key^{+}$) while maximizing the cosine distances between query and negative samples~\citep{chen2022contrastive}, 5) The recent advanced FOA~\citep{niu2024test} which uses evolution strategy to minimize the test-training statistic discrepancy and model prediction entropy.}



\subsection{Empirical observation on EM's Failure mode}
We begin by testing EM in standard TTA setting~\citep{wang2020tent}, and put forward the following observations to explain its unsatisfying performance.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/motivation.png}
    \caption{Comparison on two representative TTA methods, i.e., the seminal Tent~\citep{wang2020tent} and recent SOTA SAR~\citep{niu2023towards}, where the test dataset is ImageNet-C, snow corruption, severity level 5. We equip EM and the proposed \texttt{COME} to these two methods and observe their behaviors respectively. Along the TTA process, the uncertainty of models tuned with EM quickly drops, and the false positive rate decreases temporarily for a very short time horizon before quickly increasing. Along the same adaption trajectory, the model accuracy also improves for a short time compared to the initial model and then quickly collapse, after which the model collapses to a trivial solution. By contrast, our \texttt{COME} establishes a stable TTA process with consistently improved classification accuracy and false positive rate. Besides, the model confidence of our \texttt{COME} is much more conservative, which implies fewer risks of overconfidence and a more accurate uncertainty awareness.}
    \label{fig:motivation2}
    \vspace{-20pt}
\end{figure}

As shown in Figure~\ref{fig:motivation1} and~\ref{fig:motivation2}, after TTA, EM tends to overconfident prediction and assign all the probability to one certain class. While we believe that tuning the model to favor confident prediction can boost classification accuracy, the unlimited low entropy on all test samples is absolutely a rather undesired feature. The most straightforward way to overcome this limitation is to filter out unreliable samples. In Figure~\ref{fig:motivation1}, we try to stable TTA by filtering out the unreliable samples with high entropy and only conducting EM on the rest $m\%$ low-entropy samples. However, the resultant method still suffers from overconfidence and model collapse issues, which urges the demand of more effective methods. These observations motivates the proposal of our \texttt{COME} to explicitly models uncertainty and regularize the model for conservative predictive confidence during TTA.



==> sections/theory.tex <==
\section{Theory}
In this section, we provide theoretical understanding of the superiority of UEM. At a high level, we prove our method is a realization of Maximum A Posteriori (MAP) estimation in Bayesian statistic. Besides, compared to traditional EM methods pursue prediction with absolutely low entropy, the predicted entropy of UEM is lower bounded in a data-adapt manner and thus avoids uncertainty collapse. To introduce the theoretical framework, we first present the basic settings.

\textbf{Connection to MAP estimation.} We present our main result that our UEM can be considered as a realization of MAP in Bayesian statistic. Assume that we want to estimate the true class probability $\mu(x)$ for sample $x$. In supervised learning task, $\mu$ can be estimated on the observation $y$. The function $ p(y|\mu,x)$ is known as the likelihood function and the estimate $\hat{\mu}(x)=\arg\max_{\mu} f(y|\mu,x)$ is the Maximum Likelihood Estimate (MLE) of $\mu$. However, due to the unsupervised fact of TTA, the true label $y$ is inaccessible, and we can only leverage the pretrain model $f_{\theta_0}$ at hand. The most intuitive solution is to simply consider the predicted label $\hat{y}=f_{\theta_0}(x)$ as the true label (i.e., the pseudo label) and then employ the standard cross-entropy loss $\mathcal{L}_{\rm PL}=-\log \mu_{\hat{y}}(x)$. Alternatively, one can also use entropy minimization, which inherently boosts the likelihood of a few most probable classes by minimizing $\mathcal{L}_{\rm EM}=-\sum_{k=1}^K\mu_k \log \mu_{k}$.

Now assume that there exists a prior distribution $p(\mu)$ over $\mu$. This allow us to treat $\mu$ as a random variable as in Bayesian statistics. Given the true label $y$, we can calculate the posterior distribution $\mu$ using Bayes' theorem as follow
\begin{equation}
    p(\mu|y,x)=\frac{p(y|\mu,x)p(\mu|x)p(x)}{p(y,x)}\propto p(y|\mu,x)p(\mu).
\end{equation}
The method of Maximum A Posteriori (MAP) estimation then estimate $\mu$ as the mode of the posterior distribution by
\begin{equation}
    \hat{\mu}=\arg\max_{\mu} p(\mu|y,x)=\arg\max_{\mu}\ \underbrace{p(y|\mu,x)}_{\rm likelihood}\ \underbrace{p(\mu)}_{\rm prior}.
\end{equation}
MAP estimation can therefore be seen as a regularization of MLE, which expects the estimated $\hat{\mu}$ not only maximize the likelihood, but also the prior. As mentioned before, due to the inaccessibility of $y$, maximizing the likelihood can be heuristically replaced by pseudo label or entropy minimization algorithms. We then consider the prior and prove that it can be bounded by constraining on the total uncertainty mass $\mu$ as we devised in our UEM. This theorem is formally presented as
\begin{theorem}
\label{theorem:map}
For any $x\in\mathcal{X}$, assuming the prior distribution $p(\mu)$ over $\mu$ is a Dirichlet of which the parameters $\alpha$ are all equal, then we have
\begin{equation}
    -\log p(\mu) \leq (S_0-K)(K^{-1/2}+1)u^{-1}(x)+{\rm const},
\end{equation}
where $S_0\geq K$ is the strength of the Dirichlet prior, $K$ is the number of total classes. $\mu$ is the predicted class distribution and $u(x)$ is the uncertainty mass as defined in Eq.~\ref{SL}.
\end{theorem}
The proof is deferred to the Appendix. Theorem.~\ref{theorem:map} illustrates that the total uncertainty mass in our UEM is positively related to the Dirichlet prior over the prediction $\mu$. Thus constrain on $u(x)$ i.e., encouraging $u$ to decrease or at least not increase too much is equivalent to maximize the prior. In Theorem~\ref{theorem:map}, a flat Dirichlet is chosen as the prior distribution in accordance with the principle of insufficient reason~\cite{murphy2012machine}, where all possible categorical distributions $\mu$ are equiprobable.

\textbf{Stability of UEM.} We now investigate another essential property of UEM to explain why it can help to stabilize TTA. One limitation of EM is that it enforces unbounded low-entropy. Our UEM resolves this issue and assigns a low-bounded entropy for each $x$ in a data-adaptive manner. This property is formalized as follow
\begin{theorem}
\label{theorem:ent-lb}
For any $x\in\mathcal{X}$, if $|u(x)- u_0(x)|\leq \delta$, then we have
    \begin{equation}
        H(\mathcal{\mu}(x))\geq -(1+\delta-u_0(x))\log (1+\delta-u_0).
    \end{equation}
\end{theorem}
From Theorem~\ref{theorem:ent-lb}, we find that the softmax entropy in UEM has a sample-wise lower bound for each $x$. In particular, it implies that the lower bound of the loss value increases with the value of $u(x)$. The high lower bound can cause optimization difficulty. For this reason, one can suspect that if the pretrain model is uncertain about some sample $x$, it will pay more attention on optimization on other more reliable samples instead, which is a desirable property for TTA in the wild.

==> sections/theory_v2.tex <==
\section{Theory}
In this section, we provide theoretical understanding of the superiority of UEM. As we mentioned before, one notable limitation of EM is that it enforces low-entropy for all test samples while ignores the instinct complexity of wild test data. Thus at the end of TTA progress, EM ultimately produces models that yields one-hot class probability with entropy nearly to zero. Our UEM resolves this issue and introduces an entropy lower bound for each $x$ according to its trustworthiness. This property is formalized as follow
\begin{theorem}
\label{theorem:ent-lb}
For any $x\in\mathcal{X}$, if $|u(x)- u_0(x)|\leq \delta$, then we have
    \begin{equation}
        H(\mathcal{\mu}(x))\geq -(1+\delta-u_0(x))\log (1+\delta-u_0).
    \end{equation}
\end{theorem}
From Theorem~\ref{theorem:ent-lb}, we find that the softmax entropy in UEM has a sample-wise lower bound for each $x$. In particular, it implies that the lower bound of the loss value increases with the value of $u(x)$. The high lower bound can cause optimization difficulty. For this reason, one can suspect that if the pretrain model is uncertain about some sample $x$, it will pay more attention on optimization on other more reliable samples instead, which is a desirable property for TTA in the wild.

==> sections/tmp.tex <==
We then formalize all possible distributions that the model might encounter.

\begin{itemize}
\item Covariant-shifted data $P^{\rm COV}_{\mathcal{XY}}$ which is relevant to model generalization. $\mathcal{P}^{\rm COV}_{\mathcal{XY}}$ is of the same label space with ID. However, its marginal distribution $P^{\rm COV}_{\mathcal{X}}$ encounters shifts due to unexpected noise or corruption.
\item Semantic-shifted outliers $\mathcal{\mathcal{P}^{\rm SEM}_{\mathcal{XY'}}}$ is the distribution of abnormal data that do not belong to any known class. Its label space has no overlap with the known label space, i.e., $\mathcal{Y'}\cap\mathcal{Y}=\emptyset$.
\end{itemize}

In this paper, we consider open world TTA setting, where $P^{test}$ is a mixture of covariant-shifted data and semantic-shifted outliers, i.e., $P^{test}=\pi P^{Cov}+(1-\pi)P^{Sem}$. We omit the subscript for simplification.


The goal of error detection is to build a detector $G:\mathcal{X}\rightarrow {\rm [Wrong, Right]}$ to predict whether the prediction is prone to be wrong through a thresholding comparison
\begin{equation}
    G_{\gamma}(x)=\left\{
\begin{aligned}
&{\rm Wrong}\ &U(x)> \gamma\\
&{\rm Right}\ &U(x)\leq\gamma
\end{aligned}
\right.\ ,
\end{equation}
where $\gamma$ is the threshold. $U(x)$ is the uncertainty scoring function deduced from $f$, which is expected to assign a higher value to the mis-classified samples. The metric we used are summarized as follow
\begin{itemize}
    \item Classification accuracy (Acc$\uparrow$) := $\mathbb{E}_{(x,y)\sim P^{test}}\mathbb{I}(\arg\max_k p(x)=y)$ which is a standard measurement of model generalization performance.
    \item False positive rate (FPR$\downarrow$) := $\mathbb{E}_{\tilde{x}}(\mathbb{I}(G_{\gamma}(\tilde{x})={\rm Right}))$ measures the error detection ability, where $\gamma$ is chosen when true positive rate (TPR) is $95\%$. $\mathbb{I}$ is the indicator function. $\tilde{x}$ denotes the mis-classified samples. Higher FPR indicates that the model assign low uncertainty on even mis-classified samples and thus it is untrustworthy.
\end{itemize}



\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.99\textwidth]{figs/openworld.png}
    \caption{Models trained on in-distribution (ID) data (left) inevitably encounter distributional shifts during their deployment. Entropy minimization (EM) expects the model to correctly classify covariate-shifted data that undergoes noise or corruption by continuously minimizing the model uncertainty at inference time. However, this learning principle ignores the instinct complexity of sample, where there always exists irreducible uncertainty raises upon unreliable samples (grey area in the middle figure) that lie near the decision boundary or abnormal outliers (pink samples in the right figure) that do not belong to any known classes. Naturally, we expect the model to express relatively high uncertainty on erroneous predictions or abnormal outliers for trustworthiness.}
    \label{fig:openworld}
\end{figure}

==> tabs/tab-ood.tex <==
\begin{table}[!htbp]
    \centering
    \caption{Classification and uncertainty estimation comparisons with SOTA methods on ImageNet-C under open-world TTA settings. $P^{\rm test}$ is a mixture of both normal covariate-shifted test samples and abnormal outliers, i.e., $P^{\rm test}=\pi P^{\rm Cov}+(1-\pi)P^{\rm Sem}$, $\pi=0.5$. Full results with standard deviation and various $\pi$ are in the Appendix.}
    \label{tab:ood detection performance on each OOD dataset imagenet}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cc|cc|cc|cc|cc|cc|cc|cc|cc}
    \toprule
     & & \multicolumn{10}{c}{Natural Outliers Exposure} & \multicolumn{4}{c}{Adversarial Attack} & &   \\ 
    \cmidrule(r){3-12} \cmidrule(r){13-16} \cmidrule(r){17-18}    
     Methods & CML & \multicolumn{2}{c}{NINCO} & \multicolumn{2}{c}{iNaturist} & \multicolumn{2}{c}{SSB-Hard} & \multicolumn{2}{c}{Texture} & \multicolumn{2}{c}{Places} & \multicolumn{2}{c}{FGSM} & \multicolumn{2}{c}{PGD} & \multicolumn{2}{c}{Avg.} \\ & & Acc. &FPR. & Acc. &FPR. & Acc. &FPR. & Acc. &FPR. & Acc. &FPR. & Acc. &FPR. & Acc. &FPR. & Acc. &FPR. \\


\midrule \multirow{3}{*}{tent+level3}
&\xmark   &62.56&71.65&36.50&90.46&65.27&78.13&64.24&66.59&45.97&85.70&46.03&74.99&56.73&76.12&53.90&77.66\\
&\cmark  &65.02&64.66&71.90&67.33&69.80&73.32&65.83&58.40&26.29&30.91&47.28&70.79&60.44&71.58&58.08&62.43\\
&Improve  &\textcolor{mycolor4}{$\bigtriangleup2.47$} &\textcolor{mycolor4}{$\bigtriangledown7.00$} &\textcolor{mycolor4}{$\bigtriangleup35.41$} &\textcolor{mycolor4}{$\bigtriangledown23.13$} &\textcolor{mycolor4}{$\bigtriangleup4.53$} &\textcolor{mycolor4}{$\bigtriangledown4.81$} &\textcolor{mycolor4}{$\bigtriangleup1.60$} &\textcolor{mycolor4}{$\bigtriangledown8.19$} &\textcolor{mycolor3}{$\bigtriangledown19.68$} &\textcolor{mycolor4}{$\bigtriangledown54.79$} &\textcolor{mycolor4}{$\bigtriangleup1.25$} &\textcolor{mycolor4}{$\bigtriangledown4.20$} &\textcolor{mycolor4}{$\bigtriangleup3.71$} &\textcolor{mycolor4}{$\bigtriangledown4.54$} &\textcolor{mycolor4}{$\bigtriangleup4.18$} &\textcolor{mycolor4}{$\bigtriangledown15.24$} \\

\midrule \multirow{3}{*}{tent+level5}
&\xmark   &43.62&80.17&25.90&92.19&50.34&81.86&44.22&78.48&22.19&92.88&2.66&98.45&20.79&91.35&29.96&87.91\\
&\cmark  &45.76&78.08&44.98&67.12&53.42&81.52&46.28&77.31&13.03&51.62&15.16&51.10&15.32&43.28&33.42&64.29\\
&Improve  &\textcolor{mycolor4}{$\bigtriangleup2.14$} &\textcolor{mycolor4}{$\bigtriangledown2.08$} &\textcolor{mycolor4}{$\bigtriangleup19.08$} &\textcolor{mycolor4}{$\bigtriangledown25.07$} &\textcolor{mycolor4}{$\bigtriangleup3.08$} &\textcolor{mycolor4}{$\bigtriangledown0.34$} &\textcolor{mycolor4}{$\bigtriangleup2.06$} &\textcolor{mycolor4}{$\bigtriangledown1.16$} &\textcolor{mycolor3}{$\bigtriangledown9.16$} &\textcolor{mycolor4}{$\bigtriangledown41.27$} &\textcolor{mycolor4}{$\bigtriangleup12.50$} &\textcolor{mycolor4}{$\bigtriangledown47.35$} &\textcolor{mycolor3}{$\bigtriangledown5.48$} &\textcolor{mycolor4}{$\bigtriangledown48.08$} &\textcolor{mycolor4}{$\bigtriangleup3.46$} &\textcolor{mycolor4}{$\bigtriangledown23.62$} \\

    \bottomrule
    \end{tabular}
    }
    \end{table}
    

==> tabs/tab-standard-acc-backup.tex <==
\begin{table}[htbp]
\centering
\caption{Classification performance and uncertainty estimation comparison on ImageNet-C. Substantial ($\geq 0.5$) \textcolor{mycolor4}{improvement} and \textcolor{mycolor3}{degradation} compared to the baseline are highlighted in blue or red respectively. The \textbf{best} and \underline{second-best} results are in bold or underlined. TTA methods equipped with \texttt{COME} consistently surpass their counterparts. Full results with standard deviation are in the Appendix.}
\label{tab:ood detection performance on each OOD dataset imagenet}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{1mm}
\begin{tabular}{cc|ccc|cccc|cccc|cccc|c}
\toprule
 & & \multicolumn{3}{c}{Noise} & \multicolumn{4}{c}{Blur} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Digital} & \multicolumn{1}{c}{}  \\ 
\cmidrule(r){3-5} \cmidrule(r){6-9} \cmidrule(r){10-13} \cmidrule(r){14-17} \cmidrule(r){18-18}  
 Methods & UEM & Gauss. & Shot & Impul. & Defoc & Glass & Motion & Zoom & Snow & Frost &Fog & Brit. &Contr. &Elast. &Pixel & JPEG & Avg. \\
 \toprule
\multicolumn{18}{c}{\cellcolor{gray!20}Classification performance (Accuracy$\uparrow$)}\\
 \midrule 
No Adapt
& N/A &35.1 & 32.2 & 35.9 & 31.4 & 25.3 & 39.4 & 31.6 & 24.5 & 30.1 & 54.7 & 64.5 & 49.0 & 34.2 & 53.2 & 56.5 & 39.8\\
 \midrule 
PL
& N/A &49.9 & 48.6 & 51.1 & 48.0 & 41.0 & 52.8 & 43.1 & 22.6 & 40.7 & 63.8 & 73.0 & 65.4 & 43.5 & 63.9 & 62.7 & 51.3\\

T3A (~\cite{iwasawa2021test})
& N/A &34.5 & 31.5 & 35.4 & 32.6 & 27.5 & 40.8 & 33.6 & 25.7 & 31.0 & 56.4 & 64.9 & 50.8 & 37.9 & 54.3 & 58.4 & 41.0\\

TEA (~\cite{yuan2023energy})
& N/A &44.6 & 39.2 & 45.9 & 38.0 & 36.0 & 46.5 & 38.4 & 9.1 & 46.7 & 59.9 & 72.3 & 59.9 & 45.6 & 62.4 & 59.0 & 46.9\\
LAME
& N/A &34.8 & 31.9 & 35.5 & 31.0 & 24.4 & 39.0 & 30.7 & 23.4 & 29.6 & 53.3 & 64.2 & 40.9 & 32.7 & 52.8 & 56.0 & 38.7\\

\midrule \multirow{3}{*}{TENT (~\cite{wang2020tent})}
&\xmark   &52.6 & 52.1 & 53.5 & 52.9 & 47.7 & 56.7 & 47.5 & 10.5 & 28.6 & 67.2 & 74.4 & 67.3 & 50.7 & 66.3 & 64.6 & 52.8\\
&\cmark  &53.9 & 53.9 & 55.3 & 55.9 & 51.9 & 59.8 & 52.6 & 58.7 & 61.2 & 71.3 & 78.2 & 68.9 & 58.0 & 70.5 & 68.2 & 61.2\\
&Improve  &\textcolor{mycolor4}{$\bigtriangleup1.2$} & \textcolor{mycolor4}{$\bigtriangleup1.8$} & \textcolor{mycolor4}{$\bigtriangleup1.8$} & \textcolor{mycolor4}{$\bigtriangleup3.1$} & \textcolor{mycolor4}{$\bigtriangleup4.3$} & \textcolor{mycolor4}{$\bigtriangleup3.1$} & \textcolor{mycolor4}{$\bigtriangleup5.1$} & \textcolor{mycolor4}{$\bigtriangleup48.2$} & \textcolor{mycolor4}{$\bigtriangleup32.5$} & \textcolor{mycolor4}{$\bigtriangleup4.1$} & \textcolor{mycolor4}{$\bigtriangleup3.8$} & \textcolor{mycolor4}{$\bigtriangleup1.6$} & \textcolor{mycolor4}{$\bigtriangleup7.3$} & \textcolor{mycolor4}{$\bigtriangleup4.2$} & \textcolor{mycolor4}{$\bigtriangleup3.6$} & \textcolor{mycolor4}{$\bigtriangleup8.4$}\\
\midrule \multirow{3}{*}{MEMO (~\cite{zhang2022memo})}
&\xmark   &38.7 & 35.8 & 39.1 & 31.9 & 25.5 & 39.7 & 34.2 & 26.6 & 32.0 & 53.0 & 65.3 & 54.9 & 35.2 & 55.1 & 57.7 & 41.6\\
&\cmark  &39.5 & 36.6 & 39.6 & 33.0 & 26.2 & 40.3 & 34.7 & 27.7 & 32.8 & 54.1 & 66.1 & 54.4 & 35.8 & 56.2 & 58.5 & 42.4\\
&Improve  &\textcolor{mycolor4}{$\bigtriangleup0.7$} & \textcolor{mycolor4}{$\bigtriangleup0.8$} & \textcolor{mycolor4}{$\bigtriangleup0.4$} & \textcolor{mycolor4}{$\bigtriangleup1.1$} & \textcolor{mycolor4}{$\bigtriangleup0.6$} & \textcolor{mycolor4}{$\bigtriangleup0.7$} & \textcolor{mycolor4}{$\bigtriangleup0.6$} & \textcolor{mycolor4}{$\bigtriangleup1.1$} & \textcolor{mycolor4}{$\bigtriangleup0.8$} & \textcolor{mycolor4}{$\bigtriangleup1.1$} & \textcolor{mycolor4}{$\bigtriangleup0.8$} & \textcolor{mycolor3}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangleup0.7$} & \textcolor{mycolor4}{$\bigtriangleup1.1$} & \textcolor{mycolor4}{$\bigtriangleup0.8$} & \textcolor{mycolor4}{$\bigtriangleup0.7$}\\
\midrule \multirow{3}{*}{EATA (~\cite{niu2022efficient})}
&\xmark   &55.7 & 56.5 & 57.2 & 57.3 & 53.2 & 58.3 & 58.6 & 61.8 & 60.1 & 71.1 & 75.3 & 68.5 & 62.5 & 68.7 & 66.3 & 62.1\\
&\cmark  &56.2 & 56.6 & 57.2 & 58.1 & 57.6 & 62.5 & 59.5 & 65.5 & 63.9 & 72.5 & 78.1 & 69.7 & 66.5 & 72.4 & 70.7 & 64.5\\
&Improve  &\textcolor{mycolor4}{$\bigtriangleup0.5$} & \textcolor{mycolor4}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangleup0.0$} & \textcolor{mycolor4}{$\bigtriangleup0.9$} & \textcolor{mycolor4}{$\bigtriangleup4.3$} & \textcolor{mycolor4}{$\bigtriangleup4.2$} & \textcolor{mycolor4}{$\bigtriangleup0.9$} & \textcolor{mycolor4}{$\bigtriangleup3.7$} & \textcolor{mycolor4}{$\bigtriangleup3.8$} & \textcolor{mycolor4}{$\bigtriangleup1.4$} & \textcolor{mycolor4}{$\bigtriangleup2.8$} & \textcolor{mycolor4}{$\bigtriangleup1.2$} & \textcolor{mycolor4}{$\bigtriangleup4.0$} & \textcolor{mycolor4}{$\bigtriangleup3.8$} & \textcolor{mycolor4}{$\bigtriangleup4.4$} & \textcolor{mycolor4}{$\bigtriangleup2.4$}\\
\midrule \multirow{3}{*}{SAR (~\cite{niu2023towards})}
&\xmark   &51.8 & 51.7 & 52.9 & 50.8 & 48.6 & 55.3 & 49.2 & 23.3 & 46.5 & 65.6 & 73.0 & 65.8 & 51.1 & 64.0 & 62.6 & 54.2\\
&\cmark  &56.3 & 56.5 & 57.4 & 58.6 & 57.0 & 62.8 & 58.4 & 65.2 & 64.3 & 72.8 & 78.5 & 69.6 & 64.3 & 71.9 & 69.6 & 64.2\\
&Improve  &\textcolor{mycolor4}{$\bigtriangleup4.5$} & \textcolor{mycolor4}{$\bigtriangleup4.8$} & \textcolor{mycolor4}{$\bigtriangleup4.5$} & \textcolor{mycolor4}{$\bigtriangleup7.8$} & \textcolor{mycolor4}{$\bigtriangleup8.3$} & \textcolor{mycolor4}{$\bigtriangleup7.5$} & \textcolor{mycolor4}{$\bigtriangleup9.2$} & \textcolor{mycolor4}{$\bigtriangleup42.0$} & \textcolor{mycolor4}{$\bigtriangleup17.8$} & \textcolor{mycolor4}{$\bigtriangleup7.2$} & \textcolor{mycolor4}{$\bigtriangleup5.4$} & \textcolor{mycolor4}{$\bigtriangleup3.9$} & \textcolor{mycolor4}{$\bigtriangleup13.2$} & \textcolor{mycolor4}{$\bigtriangleup7.9$} & \textcolor{mycolor4}{$\bigtriangleup7.0$} & \textcolor{mycolor4}{$\bigtriangleup10.1$}\\
\midrule \multirow{3}{*}{CoTTA (~\cite{wang2022continual})}
&\xmark   &40.6 & 37.8 & 41.7 & 33.7 & 29.5 & 43.8 & 35.6 & 38.1 & 43.3 & 59.2 & 70.5 & 59.3 & 40.1 & 57.9 & 59.7 & 46.1\\
&\cmark  &43.5 & 41.4 & 45.4 & 36.8 & 29.6 & 47.6 & 38.2 & 42.1 & 42.7 & 62.4 & 73.4 & 62.9 & 43.0 & 63.2 & 63.7 & 49.1\\
&Improve  &\textcolor{mycolor4}{$\bigtriangleup2.9$} & \textcolor{mycolor4}{$\bigtriangleup3.6$} & \textcolor{mycolor4}{$\bigtriangleup3.7$} & \textcolor{mycolor4}{$\bigtriangleup3.1$} & \textcolor{mycolor4}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangleup3.8$} & \textcolor{mycolor4}{$\bigtriangleup2.5$} & \textcolor{mycolor4}{$\bigtriangleup4.0$} & \textcolor{mycolor3}{$\bigtriangledown0.6$} & \textcolor{mycolor4}{$\bigtriangleup3.2$} & \textcolor{mycolor4}{$\bigtriangleup2.8$} & \textcolor{mycolor4}{$\bigtriangleup3.6$} & \textcolor{mycolor4}{$\bigtriangleup2.9$} & \textcolor{mycolor4}{$\bigtriangleup5.3$} & \textcolor{mycolor4}{$\bigtriangleup4.0$} & \textcolor{mycolor4}{$\bigtriangleup3.0$}\\
\midrule \multirow{3}{*}{FOA}
&\xmark   &47.4 & 42.6 & 48.2 & 47.6 & 40.3 & 49.4 & 42.8 & 54.5 & 52.4 & 65.9 & 76.4 & 63.2 & 49.0 & 61.5 & 64.0 & 53.7\\
&\cmark  &46.0 & 43.6 & 48.3 & 47.7 & 40.3 & 49.5 & 44.0 & 53.1 & 54.6 & 66.4 & 76.2 & 63.5 & 47.9 & 61.6 & 64.2 & 53.8\\
&Improve  &\textcolor{mycolor1}{$\bigtriangledown1.3$} & \textcolor{mycolor4}{$\bigtriangleup1.0$} & \textcolor{mycolor4}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangleup0.0$} & \textcolor{mycolor4}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangleup1.3$} & \textcolor{mycolor1}{$\bigtriangledown1.4$} & \textcolor{mycolor4}{$\bigtriangleup2.3$} & \textcolor{mycolor4}{$\bigtriangleup0.5$} & \textcolor{mycolor1}{$\bigtriangledown0.2$} & \textcolor{mycolor4}{$\bigtriangleup0.3$} & \textcolor{mycolor1}{$\bigtriangledown1.2$} & \textcolor{mycolor4}{$\bigtriangleup0.2$} & \textcolor{mycolor4}{$\bigtriangleup0.2$} & \textcolor{mycolor4}{$\bigtriangleup0.1$}\\

\toprule
\multicolumn{18}{c}{\cellcolor{gray!20}Uncertainty estimation (FPR95$\downarrow$)}\\


 
\midrule No Adapt
& N/A &64.6 & 65.8 & 67.1 & 68.6 & 69.7 & 66.6 & 73.0 & 69.1 & 64.1 & 66.4 & 63.2 & 73.4 & 70.9 & 64.0 & 66.1 & 67.5\\
\midrule 
PL
& N/A &66.5 & 65.9 & 66.6 & 67.3 & 70.4 & 67.6 & 71.5 & 88.4 & 78.2 & 64.9 & 63.1 & 63.9 & 70.3 & 64.7 & 67.3 & 69.1\\

T3A (~\cite{iwasawa2021test})
& N/A &67.2 & 68.2 & 68.5 & 64.5 & 69.8 & 66.3 & 70.3 & 66.2 & 66.7 & 63.3 & 68.7 & 68.3 & 67.8 & 69.6 & 69.9 & 67.7\\

TEA (~\cite{yuan2023energy})
& N/A &67.2 & 68.3 & 67.2 & 70.0 & 69.3 & 67.1 & 68.5 & 94.0 & 65.2 & 63.9 & 62.8 & 65.2 & 65.6 & 63.7 & 65.9 & 68.3\\
LAME
& N/A &65.0 & 66.5 & 67.6 & 70.3 & 71.9 & 67.9 & 75.8 & 73.1 & 66.9 & 70.3 & 63.6 & 80.7 & 74.1 & 64.6 & 67.2 & 69.7\\

\midrule \multirow{3}{*}{TENT (~\cite{wang2020tent})}
&\xmark   &67.6 & 67.2 & 67.2 & 67.1 & 68.7 & 67.7 & 72.2 & 95.1 & 87.7 & 62.7 & 62.3 & 65.2 & 68.7 & 65.3 & 67.0 & 70.1\\
&\cmark  &65.9 & 66.5 & 67.2 & 68.1 & 69.1 & 67.5 & 70.8 & 70.6 & 65.1 & 61.7 & 63.1 & 63.9 & 67.5 & 64.4 & 65.9 & 66.5\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor4}{$\bigtriangledown0.7$} & \textcolor{mycolor3}{$\bigtriangleup0.0$} & \textcolor{mycolor3}{$\bigtriangleup1.1$} & \textcolor{mycolor3}{$\bigtriangleup0.4$} & \textcolor{mycolor4}{$\bigtriangledown0.2$} & \textcolor{mycolor4}{$\bigtriangledown1.4$} & \textcolor{mycolor4}{$\bigtriangledown24.5$} & \textcolor{mycolor4}{$\bigtriangledown22.7$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor3}{$\bigtriangleup0.8$} & \textcolor{mycolor4}{$\bigtriangledown1.3$} & \textcolor{mycolor4}{$\bigtriangledown1.3$} & \textcolor{mycolor4}{$\bigtriangledown0.9$} & \textcolor{mycolor4}{$\bigtriangledown1.1$} & \textcolor{mycolor4}{$\bigtriangledown3.6$}\\
\midrule \multirow{3}{*}{MEMO (\cite{zhang2022memo})}
&\xmark   &65.7 & 67.0 & 69.2 & 71.3 & 76.9 & 71.7 & 79.1 & 78.0 & 74.3 & 73.6 & 70.5 & 72.6 & 78.7 & 72.9 & 71.9 & 72.9\\
&\cmark  &64.0 & 65.1 & 66.4 & 69.7 & 73.7 & 69.7 & 77.4 & 75.8 & 72.1 & 73.0 & 70.9 & 72.0 & 78.0 & 71.8 & 71.1 & 71.4\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor4}{$\bigtriangledown1.9$} & \textcolor{mycolor4}{$\bigtriangledown2.7$} & \textcolor{mycolor4}{$\bigtriangledown1.6$} & \textcolor{mycolor4}{$\bigtriangledown3.2$} & \textcolor{mycolor4}{$\bigtriangledown2.0$} & \textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor4}{$\bigtriangledown2.3$} & \textcolor{mycolor4}{$\bigtriangledown2.2$} & \textcolor{mycolor4}{$\bigtriangledown0.6$} & \textcolor{mycolor3}{$\bigtriangleup0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.8$} & \textcolor{mycolor4}{$\bigtriangledown1.1$} & \textcolor{mycolor4}{$\bigtriangledown0.8$} & \textcolor{mycolor4}{$\bigtriangledown1.5$}\\
\midrule \multirow{3}{*}{EATA (\cite{niu2022efficient})}
&\xmark   &66.7 & 67.4 & 67.1 & 67.2 & 67.4 & 66.6 & 65.4 & 62.8 & 62.8 & 63.4 & 63.3 & 63.1 & 64.2 & 64.2 & 64.2 & 65.1\\
&\cmark  &63.9 & 63.7 & 63.6 & 66.6 & 67.1 & 64.8 & 66.9 & 62.5 & 61.9 & 61.2 & 61.3 & 62.6 & 64.3 & 62.0 & 64.4 & 63.8\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown2.8$} & \textcolor{mycolor4}{$\bigtriangledown3.7$} & \textcolor{mycolor4}{$\bigtriangledown3.5$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.3$} & \textcolor{mycolor4}{$\bigtriangledown1.9$} & \textcolor{mycolor3}{$\bigtriangleup1.4$} & \textcolor{mycolor4}{$\bigtriangledown0.3$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor4}{$\bigtriangledown2.2$} & \textcolor{mycolor4}{$\bigtriangledown2.0$} & \textcolor{mycolor4}{$\bigtriangledown0.6$} & \textcolor{mycolor3}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangledown2.2$} & \textcolor{mycolor3}{$\bigtriangleup0.3$} & \textcolor{mycolor4}{$\bigtriangledown1.3$}\\
\midrule \multirow{3}{*}{SAR (\cite{niu2023towards})}
&\xmark   &64.9 & 64.2 & 65.4 & 65.6 & 66.3 & 65.4 & 67.6 & 86.9 & 71.8 & 61.5 & 62.9 & 63.6 & 65.2 & 63.5 & 65.1 & 66.7\\
&\cmark  &63.1 & 63.0 & 63.9 & 66.0 & 65.8 & 65.2 & 67.4 & 62.2 & 62.1 & 60.5 & 61.2 & 63.6 & 65.8 & 63.4 & 63.9 & 63.8\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.9$} & \textcolor{mycolor4}{$\bigtriangledown1.2$} & \textcolor{mycolor4}{$\bigtriangledown1.5$} & \textcolor{mycolor3}{$\bigtriangleup0.4$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.2$} & \textcolor{mycolor4}{$\bigtriangledown0.2$} & \textcolor{mycolor4}{$\bigtriangledown24.7$} & \textcolor{mycolor4}{$\bigtriangledown9.7$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor3}{$\bigtriangleup0.0$} & \textcolor{mycolor3}{$\bigtriangleup0.6$} & \textcolor{mycolor4}{$\bigtriangledown0.1$} & \textcolor{mycolor4}{$\bigtriangledown1.2$} & \textcolor{mycolor4}{$\bigtriangledown2.9$}\\
\midrule \multirow{3}{*}{CoTTA (\cite{wang2022continual})}
&\xmark   &65.6 & 66.0 & 67.8 & 70.7 & 71.5 & 67.3 & 75.3 & 66.5 & 64.5 & 65.1 & 62.9 & 70.8 & 72.3 & 64.8 & 67.1 & 67.9\\
&\cmark  &64.4 & 65.0 & 64.6 & 69.9 & 73.1 & 66.8 & 76.3 & 69.9 & 68.2 & 64.9 & 62.6 & 64.4 & 74.0 & 63.3 & 65.5 & 67.5\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.2$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor4}{$\bigtriangledown3.2$} & \textcolor{mycolor4}{$\bigtriangledown0.8$} & \textcolor{mycolor3}{$\bigtriangleup1.5$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor3}{$\bigtriangleup1.0$} & \textcolor{mycolor3}{$\bigtriangleup3.3$} & \textcolor{mycolor3}{$\bigtriangleup3.7$} & \textcolor{mycolor4}{$\bigtriangledown0.1$} & \textcolor{mycolor4}{$\bigtriangledown0.3$} & \textcolor{mycolor4}{$\bigtriangledown6.4$} & \textcolor{mycolor3}{$\bigtriangleup1.7$} & \textcolor{mycolor4}{$\bigtriangledown1.5$} & \textcolor{mycolor4}{$\bigtriangledown1.5$} & \textcolor{mycolor4}{$\bigtriangledown0.3$}\\
\midrule \multirow{3}{*}{FOA}
&\xmark   &65.6 & 65.0 & 65.4 & 66.3 & 65.4 & 63.9 & 68.1 & 60.2 & 62.1 & 60.2 & 61.3 & 60.6 & 63.7 & 62.1 & 63.6 & 63.6\\
&\cmark  &65.1 & 64.1 & 65.7 & 66.1 & 66.1 & 65.2 & 66.5 & 60.1 & 60.2 & 61.5 & 61.4 & 60.0 & 64.1 & 62.8 & 63.6 & 63.5\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.9$} & \textcolor{mycolor1}{$\bigtriangleup0.3$} & \textcolor{mycolor4}{$\bigtriangledown0.2$} & \textcolor{mycolor1}{$\bigtriangleup0.7$} & \textcolor{mycolor1}{$\bigtriangleup1.2$} & \textcolor{mycolor4}{$\bigtriangledown1.5$} & \textcolor{mycolor4}{$\bigtriangledown0.1$} & \textcolor{mycolor4}{$\bigtriangledown2.0$} & \textcolor{mycolor1}{$\bigtriangleup1.3$} & \textcolor{mycolor1}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangledown0.6$} & \textcolor{mycolor1}{$\bigtriangleup0.4$} & \textcolor{mycolor1}{$\bigtriangleup0.7$} & \textcolor{mycolor1}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangledown0.1$}\\
\bottomrule
\end{tabular}
}
\end{table}


==> tabs/tab-standard-fpr.tex <==
\begin{table}[htbp]
\centering
\caption{Uncertainty estimation performance comparison on ImageNet-C. Substantial ($\geq 0.5$) \textcolor{mycolor4}{improvement} and \textcolor{mycolor3}{degradation} compared to the baseline are highlighted in blue or red respectively. The \textbf{best} and \underline{second-best} results are in bold or underlined. TTA methods equipped with UEM consistently surpass their counterparts. Full results with standard deviation are in the Appendix.}
\label{tab:ood detection performance on each OOD dataset imagenet}
\resizebox{\textwidth}{!}{
\setlength{\tabcolsep}{1mm}
\begin{tabular}{cc|ccc|cccc|cccc|cccc|c}
\toprule
 & & \multicolumn{3}{c}{Noise} & \multicolumn{4}{c}{Blur} & \multicolumn{4}{c}{Weather} & \multicolumn{4}{c}{Digital} & \multicolumn{1}{c}{}  \\ 
\cmidrule(r){3-5} \cmidrule(r){6-9} \cmidrule(r){10-13} \cmidrule(r){14-17} \cmidrule(r){18-18}  
 Methods & UEM & Gauss. & Shot & Impul. & Defoc & Glass & Motion & Zoom & Snow & Frost &Fog & Brit. &Contr. &Elast. &Pixel & JPEG & Avg. \\


 
\midrule No Adapt
& N/A &64.6 & 65.8 & 67.1 & 68.6 & 69.7 & 66.6 & 73.0 & 69.1 & 64.1 & 66.4 & 63.2 & 73.4 & 70.9 & 64.0 & 66.1 & 67.5\\
\midrule 
PL
& N/A &66.5 & 65.9 & 66.6 & 67.3 & 70.4 & 67.6 & 71.5 & 88.4 & 78.2 & 64.9 & 63.1 & 63.9 & 70.3 & 64.7 & 67.3 & 69.1\\

T3A
& N/A &67.2 & 68.2 & 68.5 & 64.5 & 69.8 & 66.3 & 70.3 & 66.2 & 66.7 & 63.3 & 68.7 & 68.3 & 67.8 & 69.6 & 69.9 & 67.7\\

TEA
& N/A &67.2 & 68.3 & 67.2 & 70.0 & 69.3 & 67.1 & 68.5 & 94.0 & 65.2 & 63.9 & 62.8 & 65.2 & 65.6 & 63.7 & 65.9 & 68.3\\

\midrule \multirow{3}{*}{TENT}
&\xmark   &67.6 & 67.2 & 67.2 & 67.1 & 68.7 & 67.7 & 72.2 & 95.1 & 87.7 & 62.7 & 62.3 & 65.2 & 68.7 & 65.3 & 67.0 & 70.1\\
&\cmark  &65.9 & 66.5 & 67.2 & 68.1 & 69.1 & 67.5 & 70.8 & 70.6 & 65.1 & 61.7 & 63.1 & 63.9 & 67.5 & 64.4 & 65.9 & 66.5\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor4}{$\bigtriangledown0.7$} & \textcolor{mycolor3}{$\bigtriangleup0.0$} & \textcolor{mycolor3}{$\bigtriangleup1.1$} & \textcolor{mycolor3}{$\bigtriangleup0.4$} & \textcolor{mycolor4}{$\bigtriangledown0.2$} & \textcolor{mycolor4}{$\bigtriangledown1.4$} & \textcolor{mycolor4}{$\bigtriangledown24.5$} & \textcolor{mycolor4}{$\bigtriangledown22.7$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor3}{$\bigtriangleup0.8$} & \textcolor{mycolor4}{$\bigtriangledown1.3$} & \textcolor{mycolor4}{$\bigtriangledown1.3$} & \textcolor{mycolor4}{$\bigtriangledown0.9$} & \textcolor{mycolor4}{$\bigtriangledown1.1$} & \textcolor{mycolor4}{$\bigtriangledown3.6$}\\
\midrule \multirow{3}{*}{MEMO}
&\xmark   &65.7 & 67.0 & 69.2 & 71.3 & 76.9 & 71.7 & 79.1 & 78.0 & 74.3 & 73.6 & 70.5 & 72.6 & 78.7 & 72.9 & 71.9 & 72.9\\
&\cmark  &64.0 & 65.1 & 66.4 & 69.7 & 73.7 & 69.7 & 77.4 & 75.8 & 72.1 & 73.0 & 70.9 & 72.0 & 78.0 & 71.8 & 71.1 & 71.4\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor4}{$\bigtriangledown1.9$} & \textcolor{mycolor4}{$\bigtriangledown2.7$} & \textcolor{mycolor4}{$\bigtriangledown1.6$} & \textcolor{mycolor4}{$\bigtriangledown3.2$} & \textcolor{mycolor4}{$\bigtriangledown2.0$} & \textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor4}{$\bigtriangledown2.3$} & \textcolor{mycolor4}{$\bigtriangledown2.2$} & \textcolor{mycolor4}{$\bigtriangledown0.6$} & \textcolor{mycolor3}{$\bigtriangleup0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.8$} & \textcolor{mycolor4}{$\bigtriangledown1.1$} & \textcolor{mycolor4}{$\bigtriangledown0.8$} & \textcolor{mycolor4}{$\bigtriangledown1.5$}\\
\midrule \multirow{3}{*}{EATA}
&\xmark   &66.7 & 67.4 & 67.1 & 67.2 & 67.4 & 66.6 & 65.4 & 62.8 & 62.8 & 63.4 & 63.3 & 63.1 & 64.2 & 64.2 & 64.2 & 65.1\\
&\cmark  &63.9 & 63.7 & 63.6 & 66.6 & 67.1 & 64.8 & 66.9 & 62.5 & 61.9 & 61.2 & 61.3 & 62.6 & 64.3 & 62.0 & 64.4 & 63.8\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown2.8$} & \textcolor{mycolor4}{$\bigtriangledown3.7$} & \textcolor{mycolor4}{$\bigtriangledown3.5$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.3$} & \textcolor{mycolor4}{$\bigtriangledown1.9$} & \textcolor{mycolor3}{$\bigtriangleup1.4$} & \textcolor{mycolor4}{$\bigtriangledown0.3$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor4}{$\bigtriangledown2.2$} & \textcolor{mycolor4}{$\bigtriangledown2.0$} & \textcolor{mycolor4}{$\bigtriangledown0.6$} & \textcolor{mycolor3}{$\bigtriangleup0.1$} & \textcolor{mycolor4}{$\bigtriangledown2.2$} & \textcolor{mycolor3}{$\bigtriangleup0.3$} & \textcolor{mycolor4}{$\bigtriangledown1.3$}\\
\midrule \multirow{3}{*}{sar}
&\xmark   &64.9 & 64.2 & 65.4 & 65.6 & 66.3 & 65.4 & 67.6 & 86.9 & 71.8 & 61.5 & 62.9 & 63.6 & 65.2 & 63.5 & 65.1 & 66.7\\
&\cmark  &63.1 & 63.0 & 63.9 & 66.0 & 65.8 & 65.2 & 67.4 & 62.2 & 62.1 & 60.5 & 61.2 & 63.6 & 65.8 & 63.4 & 63.9 & 63.8\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.9$} & \textcolor{mycolor4}{$\bigtriangledown1.2$} & \textcolor{mycolor4}{$\bigtriangledown1.5$} & \textcolor{mycolor3}{$\bigtriangleup0.4$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor4}{$\bigtriangledown0.2$} & \textcolor{mycolor4}{$\bigtriangledown0.2$} & \textcolor{mycolor4}{$\bigtriangledown24.7$} & \textcolor{mycolor4}{$\bigtriangledown9.7$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor4}{$\bigtriangledown1.7$} & \textcolor{mycolor3}{$\bigtriangleup0.0$} & \textcolor{mycolor3}{$\bigtriangleup0.6$} & \textcolor{mycolor4}{$\bigtriangledown0.1$} & \textcolor{mycolor4}{$\bigtriangledown1.2$} & \textcolor{mycolor4}{$\bigtriangledown2.9$}\\
\midrule \multirow{3}{*}{cotta}
&\xmark   &65.6 & 66.0 & 67.8 & 70.7 & 71.5 & 67.3 & 75.3 & 66.5 & 64.5 & 65.1 & 62.9 & 70.8 & 72.3 & 64.8 & 67.1 & 67.9\\
&\cmark  &64.4 & 65.0 & 64.6 & 69.9 & 73.1 & 66.8 & 76.3 & 69.9 & 68.2 & 64.9 & 62.6 & 64.4 & 74.0 & 63.3 & 65.5 & 67.5\\
&Improve  &\textcolor{mycolor4}{$\bigtriangledown1.2$} & \textcolor{mycolor4}{$\bigtriangledown1.0$} & \textcolor{mycolor4}{$\bigtriangledown3.2$} & \textcolor{mycolor4}{$\bigtriangledown0.8$} & \textcolor{mycolor3}{$\bigtriangleup1.5$} & \textcolor{mycolor4}{$\bigtriangledown0.5$} & \textcolor{mycolor3}{$\bigtriangleup1.0$} & \textcolor{mycolor3}{$\bigtriangleup3.3$} & \textcolor{mycolor3}{$\bigtriangleup3.7$} & \textcolor{mycolor4}{$\bigtriangledown0.1$} & \textcolor{mycolor4}{$\bigtriangledown0.3$} & \textcolor{mycolor4}{$\bigtriangledown6.4$} & \textcolor{mycolor3}{$\bigtriangleup1.7$} & \textcolor{mycolor4}{$\bigtriangledown1.5$} & \textcolor{mycolor4}{$\bigtriangledown1.5$} & \textcolor{mycolor4}{$\bigtriangledown0.3$}\\

\bottomrule
\end{tabular}
}
\end{table}

